A Case Study of Onboarding in Software Teams: Tasks and Strategies

Developers frequently move into new teams or environments across software companies. Their onboarding experience is correlated with productivity, job satisfaction, and other short-term and long-term outcomes. The majority of the onboarding process comprises engineering tasks such as fixing bugs or implementing small features. Nevertheless, we do not have a systematic view of how tasks influence onboarding. In this paper, we present a case study of Microsoft, where we interviewed 32 developers moving into a new team and 15 engineering managers onboarding a new developer into their team -- to understand and characterize developers' onboarding experience and expectations in relation to the tasks performed by them while onboarding. We present how tasks interact with new developers through three representative themes: learning, confidence building, and socialization. We also discuss three onboarding strategies as inferred from the interviews that managers commonly use unknowingly, and discuss their pros and cons and offer situational recommendations. Furthermore, we triangulate our interview findings with a developer survey ($N=189$) and a manager survey ($N=37$) and find that survey results suggest that our findings are representative and our recommendations are actionable. Practitioners could use our findings to improve their onboarding processes, while researchers could find new research directions from this study to advance the understanding of developer onboarding. Our research instruments and anonymous data are available at \url{https://zenodo.org/record/4455937#.YCOQCs_0lFd}

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> discussions.tex <==
% !TEX root = ./main.tex
\section{Automated Support for Onboarding}
%\textbf{Checklists and reminders.}
This study's findings inspired an onboarding support bot at \company{} with a goal to influence and streamline current onboarding practices for enabling a better new member experience. 
We created role-based checklists based on our findings in Section~\ref{sec:results} with actionable recommendations from week one to week 12.
The bot identifies the arrival of a new member based on the \textit{Person} database and dispatches the checklists to the new member, the manager, and mentors.
It sends a weekly reminder email that encourages mentors and managers to follow the checklist items to ensure a good onboarding experience.
Checklists are omitted for anonymization and will be shared in the final paper.
% All checklists are shared in the supplemental material.
Section~\ref{tab:findings_recommendations} shows that pull requests allow new members to learn and interact with the team;
furthermore, they are opportunities to give positive feedback to new members, which boosts confidence, as suggested by \textbf{A2.2} in Table~\ref{tab:findings_recommendations}.
Accordingly, the bot automatically nudges reviewers to provide timely, detailed, and more empathetic feedback when the pull request is owned by a new member.
In addition, the bot schedules onboarding sessions between the new member and the mentor by smartly sending calendar invites on certain focus days to promote early learning and encourage social interactions, as recommended by \textbf{A1.4} and \textbf{A3.1}.
Going forward, we envision to add an onboarding task recommendation capability in the bot to recommend tasks for new members based on their profile, stage of onboarding, and teams' current backlog of work items with a goal to increase their confidence (\textbf{A2.1}) and promote social interactions (\textbf{E1.2} and \textbf{A3.3}).
The bot is currently deployed for two large business groups inside \company{}, consisting of approx. 15,000 developers with a rate of about 25-30 new or transfer hires every two weeks. 

\begin{comment}
\section{Future Directions}
\label{sec:discussions}
We discuss some future directions our study suggests that could be used to improve onboarding processes.
We group the discussion into research directions and practical recommendations.

\subsection{Research directions}
\textbf{Experimentally Validating our findings.}
Our findings listed in Table~\ref{tab:findings_recommendations} and Section~\ref{sec:strategies} should be validated experimentally.
For example, in Section~\ref{sec:strategies} we hypothesize that \emph{exploration-based onboarding strategies will cause a bad onboarding experience for less experienced developers.}
Such a hypothesis could be validated more rigourously by experiments.

\textbf{Measuring onboarding tasks through artifacts.}
As a case study, our measurements of tasks are subjective.
To bridge the gap between observations and practice, we encourage future studies to design objective measurements.
Here, we propose some hypotheses:
\begin{itemize}
    \item A task's complexity can be measured by the code complexity of modules that are relevant to this task.
    \item A team member's knowledge level of a task can be measured by the history of contributions recorded by the team's task management system.
    \item A task's level of integration can be measured by the frequency of edits recorded by the code repository's version control system.
\end{itemize}
Such objective measurements could be used as building blocks of an automated onboarding support system.
\end{comment}

